Towards Open Vocabulary Learning: A Survey

In the field of visual scene understanding, deep neural networks have made impressive advancements in various core tasks like segmentation, tracking, and detection. However, most approaches operate on the close-set assumption, meaning that the model can only identify pre-defined categories that are present in the training set. Recently, open vocabulary settings were proposed due to the rapid progress of vision language pre-training. These new approaches seek to locate and recognize categories beyond the annotated label space. The open vocabulary approach is more general, practical, and effective compared to weakly supervised and zero-shot settings. This paper provides a thorough review of open vocabulary learning, summarizing and analyzing recent developments in the field. In particular, we begin by comparing it to related concepts such as zero-shot learning, open-set recognition, and out-of-distribution detection. Then, we review several closely related tasks in the case of segmentation and detection, including long-tail problems, few-shot, and zero-shot settings. For the method survey, we first present the basic knowledge of detection and segmentation in close-set as the preliminary knowledge. Next, we examine various scenarios in which open vocabulary learning is used, identifying common design elements and core ideas. Then, we compare the recent detection and segmentation approaches in commonly used datasets and benchmarks. Finally, we conclude with insights, issues, and discussions regarding future research directions. To our knowledge, this is the first comprehensive literature review of open vocabulary learning. We keep tracing related works at https://github.com/jianzongwu/Awesome-Open-Vocabulary.

==> Fig/old/3_method_review_old.tex <==
\if 0 % xsl 
\noindent
\textbf{Knowledge distillation}
Vision language models such as CLIP\cite{CLIP} are trained using large amounts of image-caption pairs, and they can recognize various objects without limiting themselves to closed vocabulary. So it is a good idea to distillate  the classification ability from VLMs to open vocabulary object detection method. ViLD\cite{gu2021open_vild} is a two-stage detection method using instance-level visual-to-visual knowledge distillation.  In the ViLD-text branch, the detection method's learnable classifier is replaced with fixed text embeddings that feed text descriptions of base categories, known as prompt, into the text encoder of VLMs. In ViLD-image branch, the pre-computed proposals are first sent to the detector to get region embeddings, and second, the proposal cropped image will be sent to image encoder of VLMs to get image embeddings. And then, ViLD-image will distill knowledge from image embeddings to region embeddings using $\mathcal L_1$ Loss. HierKD\cite{Ma2022HierKD} proposes a global-level language-to-visual knowledge distillation module to narrow the performance gap between one-stage methods and two-stage methods. The global-level knowledge distillation module(GKD) will align global-level image representations from FPN\cite{fpn} layers with caption knowledge using contrastive loss. object-centric-ovd\cite{Hanoona2022Bridging} uses inter-embedding relationship matching loss(IRM) to instill relationships within our detection region representations to be consistent with the CLIP region representations.
\fi


% xsl 
\if 0
\noindent
\textbf{Detection-tailored pretraining}
Object detection methods \cite{ren2015faster, focal_loss, detr} have achieved great success in the past decades, but these methods need a large amount of annotated data, and they can only detect object categories that the training data contains. Open vocabulary object detection aims to detect novel categories doesn't appear in the training data with the help of pre-trained VLMs. OVR-CNN\cite{zareian2021opendet_ovrcnn} first trains the ResNet\cite{resnet} and Vision to Language(V2L) layer using image-caption pairs via grounding, masked language modeling, and image-text matching. Since captions are not constraints in vocabulary, the V2L layer learns to map features from visual space into semantic space without limiting to closed vocabulary. And the pre-trained ResNet is used to initialize the backbone of Faster R-CNN\cite{ren2015faster} during the next stage of training. When learning open vocabulary detection, OVR-CNN\cite{zareian2021opendet_ovrcnn} adopts Faster R-CNN as a detection method and only replaces learnable classifier with fixed text embeddings from pre-trained language model\cite{devlin2018bert}. For classification, region visual features obtained from RoI-Align\cite{maskrcnn} are sent into the V2L layer and mapped into semantic space.  RegionCLIP\cite{Zhong2021RegionCLIPRL} learns visual region representation by matching image regions to region-level descriptions. RegionCLIP first creates region-text pairs as pseudo labels by CLIP. Given these pseudo labels, the visual encoder learns to match the region and text pairs via contrastive loss and then, the visual encoder will be fine-tuned using a human-annotated detection dataset. OWL-ViT\cite{minderer2022simple} remove the final token pooling layer of the image encoder of pre-trained VLMs and attach a lightweight classification and box head to each transformer output token and fine-tune the pre-trained model on standard detection datasets using a bipartite matching loss. 

%
\fi

\if 0
\noindent
\textbf{Object-language alignments}
Using language as supervision instead ground truth bounding box is an attractive alternative for open vocabulary object detection. However, it is difficult and costly to get enough object-language annotations. VLDet\cite{VLDet} converts the image into a set of regions and the caption into a set of words, and solves the object-language alignment problem using a set matching method.
BARON\cite{wu2023baron} proposes to align the embedding of bag of regions instead of only individual regions. They first group
contextually interrelated regions as a bag and treat each region in the bag as the word in a sentence, and then send the bag of regions into the text encoder to get bag-of-regions embeddings. These bag-of-regions embeddings will align with cropped region embeddings from image encoder of VLMs. The F-VLM\cite{Kuo2022FVLMOO} is a simple two-branch method similar to ViLD-text\cite{gu2021open_vild} during training. But the backbone of F-VLM is initialized using CLIP image encoder and frozen. During inference, F-VLM will apply the VLM feature pooler on the region features from frozen backbones and get VLM predictions using region pooling features. And the final result of F-VLM will combine the detection scores and the VLM predictions. 
\fi


\if 0
\noindent
\textbf{Prompt engineering of text encoder}
Instead of focusing on the classification of object detection methods, DetPro\cite{Du2022LearningTP} and PromptDet\cite{feng2022promptdet} turn eyes on prompt engineering of the text encoder. It is inspired by the recent progress of prompt representation learning, e.g, CoOp\cite{zhou2022coop}.  The text embeddings of category names are generated by feeding prompts to the text encoder of pre-trained VLMs. However, the negative proposals do not correspond to any specific category. OVR-CNN\cite{zareian2021opendet_ovrcnn} sets the background class to have a fixed, all-zero embedding. ViLD\cite{gu2021open_vild} use a learnable embedding to represent the background class. DetPro\cite{Du2022LearningTP} forces the negative proposal to be equally unlike any object classes instead of using the background class. PromptDet\cite{feng2022promptdet} introduces the description of the category into  the prompt and discusses the position of the category in the prompt.
\fi





\if 0

Despite the Open Vocabulary settings, there are also problems that detect/segment novel categories but do not specifically assign distinct labels to them. The novel categories are labeled as 'unknown.' Two main topics are Open World Object Detection and Open-Set Panoptic Segmentation. We call these settings Class Agnostic Detection/Segmentation.

\noindent
\textbf{Open World Object Detection.}
\cite{openworld} proposes the Open World Recognition task, which requires the model to identify novel categories and label them as `unknown.' After that, the novel categories are annotated progressively. The model needs to learn incrementally with the data and identify the newly-annotated categories. Motivated by them, \cite{openworld-detection} proposes Open World Object Detection (OWOD), which expands the recognition task into a detection one. To handle the proposed problem, this paper proposes the ORE method. It utilizes contrastive clustering and an energy based unknown identification module. \cite{OW-DETR} introduces a novel end-to-end transformer-based framework, OW-DETR. It comprises three dedicated components, namely, attention-driven pseudo-labeling, novelty classification, and objectness scoring to explicitly address the OWOD challenge. \cite{Open-World-DETR} proposes a two-stage training approach named Open World DETR. It is based on Deformable DETR and focuses on alleviating catastrophic forgetting when the annotations of the unknown classes become available incrementally by using knowledge distillation and exemplar replay technologies. PROB~\cite{PROB} proposes a probabilistic objectness head into the standard deformable DETR model to handle the challenge. Recently, \cite{UC-OWOD} proposes Unknown-Classified Open
World Object Detection (UC-OWOD) aims to detect unknown instances and classify them into different unknown classes. This task is close to the Open Vocabulary setting, but further requires incremental learning.

\noindent
\textbf{Open Set Panoptic Segmentation.}
\cite{EOPSN} proposes Open-Set Panoptic Segmentation (OSPS), which requires the model to identify novel categories as `unknown' in a panoptic segmentation task. It proposes the EOPSN framework, which uses exemplar theory, to handle this task. \cite{dual} proposes a divide-and-conquer scheme to develop a dual decision process for OSPS. The paper shows that by properly combining a known class discriminator with an additional class-agnostic object prediction head, the OSPS performance can be significantly improved.
\fi
